Hierarchical Open-Vocabulary 3D Scene Graphs for Language-Grounded Robot Navigation

Recent open-vocabulary robot mapping methods enrich dense geometric maps with pre-trained visual-language features. While these maps allow for the prediction of point-wise saliency maps when queried for a certain language concept, large-scale environments and abstract queries beyond the object level still pose a considerable hurdle, ultimately limiting language-grounded robotic navigation. In this work, we present HOV-SG, a hierarchical open-vocabulary 3D scene graph mapping approach for language-grounded robot navigation. Leveraging open-vocabulary vision foundation models, we first obtain state-of-the-art open-vocabulary segment-level maps in 3D and subsequently construct a 3D scene graph hierarchy consisting of floor, room, and object concepts, each enriched with open-vocabulary features. Our approach is able to represent multi-story buildings and allows robotic traversal of those using a cross-floor Voronoi graph. HOV-SG is evaluated on three distinct datasets and surpasses previous baselines in open-vocabulary semantic accuracy on the object, room, and floor level while producing a 75% reduction in representation size compared to dense open-vocabulary maps. In order to prove the efficacy and generalization capabilities of HOV-SG, we showcase successful long-horizon language-conditioned robot navigation within real-world multi-storage environments. We provide code and trial video data at http://hovsg.github.io/.

==> tables/habitat_20_sem_seg.tex <==
\begin{table*}[b]
\centering
\scriptsize
\caption{3D Semantic Segmentation on \\ 20 Frequent Categories on HM3DSem}
\setlength\tabcolsep{3pt}
\begin{threeparttable}
\begin{tabular}{cc|ccc}
 \toprule

Method & Scene  & $\text{mIOU}$ & $\text{F-mIOU}$ & $\text{mAcc}$  \\
\midrule

% \multirow{8}{*}{\rotatebox[origin=c]{90}{ConceptGraphs~\cite{conceptgraphs}}} & \textit{00824} & 39.34 & 58.66 & 45.60 \\ % sunny-pond
% & \textit{00829} & 29.03 & 31.35 & 38.00  \\ % sunny-pond
% & \textit{00843} & 30.10 & 33.43 & 37.56  \\ % sunny-pond
% & \textit{00861} & 26.79 & 39.73 & 35.94   \\ % sunny-pond
% & \textit{00862} & 33.71 & 34.24 & 42.36   \\ % desert-yoghurt
% & \textit{00873} & 40.27 & 61.36 & 44.31   \\ % lilac-bird
% & \textit{00877} & 52.58 & 78.83 & 57.72   \\ % lilac-bird
% & \textit{00890} & 31.32 & 51.12 & 40.95   \\ % ethereal-meadow
% \cmidrule{2-5}
% \multicolumn{2}{r|}{Overall}  & 27.79 & 41.99 & 37.48  \\
\multirow{8}{*}{\rotatebox[origin=c]{90}{ConceptGraphs~\cite{conceptgraphs}}} & \textit{00824} & 44.4 & 60.6 & 55.3 \\ % sunny-pond
& \textit{00829} & 52.7 & 51.2 & 62.0  \\ % sunny-pond
& \textit{00843} & 39.9 & 43.6 & 43.8  \\ % sunny-pond
& \textit{00861} & 34.3 & 47.1 & 45.2   \\ % sunny-pond
& \textit{00862} & 47.9 & 50.6 & 56.6   \\ % desert-yoghurt
& \textit{00873} & 50.0 & 79.2 & 55.9   \\ % lilac-bird
& \textit{00877} & 65.5 & 87.0 & 73.4   \\ % lilac-bird
& \textit{00890} & 39.8 & 55.3 & 53.2   \\ % ethereal-meadow
\cmidrule{2-5}
\multicolumn{2}{r|}{Overall}  & 46.8 & 59.3 & 55.7  \\
 \midrule
 \multirow{8}{*}{\rotatebox[origin=c]{90}{VLMaps~\cite{huang23vlmaps} w/ LSeg}} & \textit{00824} & 39.15 & 58.62 & 45.01 \\ % sunny-pond
& \textit{00829} & 48.93 & 58.33 & 57.86  \\ % sunny-pond
& \textit{00843} & 30.65 & 42.19 & 40.96  \\ % sunny-pond
& \textit{00861} & 35.27 & 48.60 & 41.54   \\ % sunny-pond
& \textit{00862} & 40.30 & 46.59 & 46.18   \\ % desert-yoghurt
& \textit{00873} & 42.83 & 70.13 & 47.30   \\ % lilac-bird
& \textit{00877} & 48.09 & 79.34 & 52.79   \\ % lilac-bird
& \textit{00890} & 37.81 & 52.18 & 43.54   \\ % ethereal-meadow
\cmidrule{2-5}
\multicolumn{2}{r|}{Overall}  & 40.4 & 57.0 & 47.0  \\
 \midrule
%  \multirow{8}{*}{\rotatebox[origin=c]{90}{HOV-SG w/ ViT-H}} & \textit{00824} & 19.88 & 43.28 & 30.10 \\ % sunny-pond
% & \textit{00829} & 40.83 & 44.59 & 47.46  \\ % sunny-pond
% & \textit{00843} & 33.65 & 56.34 & 40.47  \\ % sunny-pond
% & \textit{00861} & 27.53 & 46.30 & 38.91   \\ % sunny-pond
% & \textit{00862} & 29.30 & 35.15 & 39.93   \\ % desert-yoghurt
% & \textit{00873} & 45.39 & 50.45 & 72.01   \\ % lilac-bird
% & \textit{00877} & 60.48 & 81.09 & 64.12   \\ % lilac-bird
% & \textit{00890} & 28.59 & 45.31 & 41.82   \\ % ethereal-meadow
% \cmidrule{2-5}
% \multicolumn{2}{r|}{Overall (ours)}  & 35.70 & 53.01 & 44.16  \\
 \multirow{8}{*}{\rotatebox[origin=c]{90}{HOV-SG w/ ViT-H}} & \textit{00824} & 31.0 & 48.8 & 45.9 \\ % 
& \textit{00829} & 43.7 & 40.2 & 58.3  \\ % 
& \textit{00843} & 38.0 & 59.5 & 50.6  \\ % 
& \textit{00861} & 24.9 & 45.0 & 36.1   \\ % 
& \textit{00862} & 31.3 & 40.8 & 47.2   \\ % 
& \textit{00873} & 37.9 & 59.6 & 48.4   \\ % 
& \textit{00877} & 56.4 & 69.8 & 69.4   \\ % 
& \textit{00890} & 32.9 & 42.8 & 40.8   \\ % 
\cmidrule{2-5}
\multicolumn{2}{r|}{Overall (ours)}  & 37.0 & 50.8 & 49.6  \\
\midrule
 \multirow{8}{*}{\rotatebox[origin=c]{90}{HOV-SG w/ OVSG}} & \textit{00824} & 33.36 & 56.85 & 44.84 \\ % sunny-pond
& \textit{00829} & 55.14 & 59.14 & 61.34  \\ % sunny-pond
& \textit{00843} & 33.92 & 59.69 & 41.05  \\ % sunny-pond
& \textit{00861} & 37.43 & 58.57 & 46.65   \\ % sunny-pond
& \textit{00862} & 37.19 & 52.97 & 48.70   \\ % desert-yoghurt
& \textit{00873} & 48.23 & 77.30 & 52.96   \\ % lilac-bird
& \textit{00877} & 42.88 & 61.03 & 55.49   \\ % lilac-bird
& \textit{00890} & 31.74 & 51.89 & 48.71   \\ % ethereal-meadow
\cmidrule{2-5}
\multicolumn{2}{r|}{Overall (ours)}  & \textbf{39.99} & \textbf{59.68} & \textbf{49.97}  \\
\midrule
\bottomrule
\end{tabular}
\end{threeparttable}
\label{tab:seg-frequent-cat}
\end{table*}
